Models of Individual Blue Stragglers

This chapter describes the current state of models of individual blue stragglers. Stellar collisions, binary mergers (or coalescence), and partial or ongoing mass transfer have all been studied in some detail. The products of stellar collisions retain memory of their parent stars and are not fully mixed. Very high initial rotation rates must be reduced by an unknown process to allow the stars to collapse to the main sequence. The more massive collision products have shorter lifetimes than normal stars of the same mass, while products between low mass stars are long-lived and look very much like normal stars of their mass. Mass transfer can result in a merger, or can produce another binary system with a blue straggler and the remnant of the original primary. The products of binary mass transfer cover a larger portion of the colour-magnitude diagram than collision products for two reasons: there are more possible configurations which produce blue stragglers, and there are differing contributions to the blended light of the system. The effects of rotation may be substantial in both collision and merger products, and could result in significant mixing unless angular momentum is lost shortly after the formation event. Surface abundances may provide ways to distinguish between the formation mechanisms, but care must be taking to model the various mixing mechanisms properly before drawing strong conclusions. Avenues for future work are outlined.

==> common.tex <==
% Bibliography and bibfile
\def\aj{AJ}%
          % Astronomical Journal
\def\actaa{Acta Astron.}%
          % Acta Astronomica
\def\araa{ARA\&A}%
          % Annual Review of Astron and Astrophys
\def\apj{ApJ}%
          % Astrophysical Journal
\def\apjl{ApJ}%
          % Astrophysical Journal, Letters
\def\apjs{ApJS}%
          % Astrophysical Journal, Supplement
\def\ao{Appl.~Opt.}%
          % Applied Optics
\def\apss{Ap\&SS}%
          % Astrophysics and Space Science
\def\aap{A\&A}%
          % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}%
          % Astronomy and Astrophysics, Supplement
\def\azh{AZh}%
          % Astronomicheskii Zhurnal
\def\baas{BAAS}%
          % Bulletin of the AAS
\def\bac{Bull. astr. Inst. Czechosl.}%
          % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{Chinese Astron. Astrophys.}%
          % Chinese Astronomy and Astrophysics
\def\cjaa{Chinese J. Astron. Astrophys.}%
          % Chinese Journal of Astronomy and Astrophysics
\def\icarus{Icarus}%
          % Icarus
\def\jcap{J. Cosmology Astropart. Phys.}%
          % Journal of Cosmology and Astroparticle Physics
\def\jrasc{JRASC}%
          % Journal of the RAS of Canada
\def\mnras{MNRAS}%
          % Monthly Notices of the RAS
\def\memras{MmRAS}%
          % Memoirs of the RAS
\def\na{New A}%
          % New Astronomy
\def\nar{New A Rev.}%
          % New Astronomy Review
\def\pasa{PASA}%
          % Publications of the Astron. Soc. of Australia
\def\pra{Phys.~Rev.~A}%
          % Physical Review A: General Physics
\def\prb{Phys.~Rev.~B}%
          % Physical Review B: Solid State
\def\prc{Phys.~Rev.~C}%
          % Physical Review C
\def\prd{Phys.~Rev.~D}%
          % Physical Review D
\def\pre{Phys.~Rev.~E}%
          % Physical Review E
\def\prl{Phys.~Rev.~Lett.}%
          % Physical Review Letters
\def\pasp{PASP}%
          % Publications of the ASP
\def\pasj{PASJ}%
          % Publications of the ASJ
\def\qjras{QJRAS}%
          % Quarterly Journal of the RAS
\def\rmxaa{Rev. Mexicana Astron. Astrofis.}%
          % Revista Mexicana de Astronomia y Astrofisica
\def\skytel{S\&T}%
          % Sky and Telescope
\def\solphys{Sol.~Phys.}%
          % Solar Physics
\def\sovast{Soviet~Ast.}%
          % Soviet Astronomy
\def\ssr{Space~Sci.~Rev.}%
          % Space Science Reviews
\def\zap{ZAp}%
          % Zeitschrift fuer Astrophysik
\def\nat{Nature}%
          % Nature
\def\iaucirc{IAU~Circ.}%
          % IAU Cirulars
\def\aplett{Astrophys.~Lett.}%
          % Astrophysics Letters
\def\apspr{Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\def\bain{Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\def\fcp{Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\def\gca{Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\def\grl{Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\def\jcp{J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\def\jgr{J.~Geophys.~Res.}%
          % Journal of Geophysics Research
\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\def\memsai{Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\def\nphysa{Nucl.~Phys.~A}%
          % Nuclear Physics A
\def\physrep{Phys.~Rep.}%
          % Physics Reports
\def\physscr{Phys.~Scr}%
          % Physica Scripta
\def\planss{Planet.~Space~Sci.}%
          % Planetary Space Science
\def\procspie{Proc.~SPIE}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

\newcommand{\gras}[1]{\mbox{\boldmath $#1$}}
\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}          }\hbox{$\frown$}}}$}}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\lsim{\lower.5ex\hbox{\ltsima}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
\def\lapp{\ifmmode\stackrel{<}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}
\def\gapp{\ifmmode\stackrel{>}{_{\sim}}\else$\stackrel{<}{_{\sim}}$\fi}

\def\msol{\,\mathrm{M}_\odot}
\def\media#1{\langle #1\rangle}
\def\kms{~{\rm km~ s}^{-1}}
\def\sigp{\sigma_{\rm P}}


\def\aapr{A\&A Rev. }
\def\apjl{ApJL }
\def\aj{AJ }
\def\apj{ApJ }
\def\pasp{PASP }
\def\spie{SPIE }
\def\apjs{ApJS }
\def\araa{ARAA }
\def\aap{A\&A }
\def\mnras{MNRAS }
\def\nat{Nature }

\newcommand{\lesssim}    {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{<}}}}%
\newcommand{\lsim}       {\lesssim}%
\newcommand{\la}         {\lesssim}% For Springer A&A compliance...
\newcommand{\gtrsim}     {\mbox{\rlap{\hbox{\lower3pt\hbox{\ensuremath{\sim}}}}\raise1.5pt\hbox{\ensuremath{>}}}}%
\newcommand{\gsim}       {\gtrsim}%
\newcommand{\ga}         {\gtrsim}%
\newcommand{\sq}         {\mbox{\rlap{\ensuremath{\sqcap}}\ensuremath{\sqcup}}}%
\newcommand{\arcdeg}     {\mbox{\ensuremath{{}^\circ}}}%
\newcommand{\arcmin}     {\mbox{\ensuremath{{}^\prime}}}%
\newcommand{\arcsec}     {\mbox{\ensuremath{{}^{\prime\prime}}}}%

% Journal abbreviations
\def\aj{\rmfamily{AJ~}}           % Astronomical Journal
\def\apj{\rmfamily{ApJ~}}         % Astrophysical Journal
\def\apjl{\rmfamily{ApJ~}}        % Astrophysical Journal, Letters
\def\apjs{\rmfamily{ApJS~}}       % Astrophysical Journal, Supplement
\let\apjlett=\apjl
\let\apjsupp=\apjs
\def\aap{\rmfamily{A\&A~}}        % Astronomy and Astrophysics
\let\astap=\aap
\def\araa{\rmfamily{ARA\&A~}}     % Annual Review of Astronomy and Astrophysics
\def\aapr{\rmfamily{A\&A~Rev.~}}  % Astronomy and Astrophysics Reviews
\def\aaps{\rmfamily{A\&AS~}}      % Astronomy and Astrophysics, Supplement
\def\mnras{\rmfamily{MNRAS~}}     % Monthly Notices of the Royal Astron. Soc.
\def\pasp{\rmfamily{PASP~}}       % Publications of the Astron. Soc. o/t Pacific
\def\apss{\rmfamily{Ap\&SS~}}     % Astrophysics and Space Science
\def\pasj{\rmfamily{PASJ~}}       % Publications of the Astron. Soc. of Japan
\def\pra{\rmfamily{Phys.~Rev.~A~}}% Physical Review A: Atomic, Molecular, and  
                                  %   Optical Physics
\def\prb{\rmfamily{Phys.~Rev.~B~}}% Physical Review B: Condensed Matter and
                                  %   Materials Physics
\def\prc{\rmfamily{Phys.~Rev.~C~}}% Physical Review C: Nuclear Physics
\def\prd{\rmfamily{Phys.~Rev.~D~}}% Physical Review D: Particles, Fields,
                                  %   Gravitation and Cosmology
\def\pre{\rmfamily{Phys.~Rev.~E~}}% Physical Review E: Statistical, Nonlinear,
                                  %   and Soft Matter Physics
\def\rmp{\rmfamily{Rev.~Mod.~Phys.~}}% Reviews of Modern Physics
\def\prl{\rmfamily{Phys.~Rev.~Lett.~}}% Physical Review Letters
\def\nat{\rmfamily{Nature~}}      % Nature
\def\sci{\rmfamily{Science~}}     % Science
\def\skytel{\rmfamily{S\&T~}}     % Sky and Telescope
\def\ao{\rmfamily{Appl.~Opt.~}}   % Applied Optics
\let\applopt=\ao
\def\azh{\rmfamily{AZh~}}         % Astronomicheskii Zhurnal
\def\baas{\rmfamily{BAAS~}}       % Bulletin of the AAS
\def\jrasc{\rmfamily{JRASC~}}     % Journal of the Royal Astron. Soc. of Canada
\def\memras{\rmfamily{MmRAS~}}    % Memoirs of the Royal Astron. Soc.
\def\qjras{\rmfamily{QJRAS~}}     % Quarterly Journal of the Royal Astron. Soc.
\def\solphys{\rmfamily{Sol.~Phys.~}}% Solar Physics
\def\sovast{\rmfamily{Soviet~Ast.~}}% Soviet Astronomy
\def\ssr{\rmfamily{Space~Sci.~Rev.~}}% Space Science Reviews
\def\zap{\rmfamily{ZAp~}}         % Zeitschrift fuer Astrophysik
\def\iauc{\rmfamily{IAU~Circ.~}}  % IAU Cirulars
\let\iaucirc=\iauc
\def\aplett{\rmfamily{Astrophys.~Lett.~}}% Astrophysics Letters
\def\apspr{\rmfamily{Astrophys.~Space~Phys.~Res.~}}% Astrophysics Space Physics
                                  % Research
\def\bain{\rmfamily{Bull.~Astron.~Inst.~Netherlands~}}% Bulletin of the 
                                  % Astronomical Institute of the Netherlands
\def\fcp{\rmfamily{Fund.~Cosmic~Phys.~}}% Fundamental Cosmic Physics
\def\gca{\rmfamily{Geochim.~Cosmochim.~Acta~}}% Geochimica Cosmochimica Acta
\def\grl{\rmfamily{Geophys.~Res.~Lett.~}}% Geophysics Research Letters
\def\jcp{\rmfamily{J.~Chem.~Phys.~}}% Journal of Chemical Physics
\def\jgr{\rmfamily{J.~Geophys.~Res.~}}% Journal of Geophysics Research
\def\jqsrt{\rmfamily{J.~Quant.~Spec.~Radiat.~Transf.~}} % Journal of Quantitative
                                  % Spectroscopy and Radiative Transfer
\def\memsai{\rmfamily{Mem.~Soc.~Astron.~Italiana~}}
                                  % Mem. Societa Astronomica Italiana
\def\nphysa{\rmfamily{Nucl.~Phys.~A~}}% Nuclear Physics A
\def\physrep{\rmfamily{Phys.~Rep.~}}% Physics Reports
\def\physscr{\rmfamily{Phys.~Scr~}}% Physica Scripta
\def\planss{\rmfamily{Planet.~Space~Sci.~}}% Planetary Space Science
\def\procspie{\rmfamily{Proc.~SPIE~}}% Proceedings of the SPIE
\def\aipconf{\rmfamily{AIP~Conf.~Proc.~}}% AIP Conference Proceedings
\def\aspconf{\rmfamily{ASP~Conf.~Ser.~}}% ASP Conference Series
\def\asslconf{\rmfamily{Ap\&SSL~Conf.~Ser.~}}% ASSL Conference Series}
\def\maps{\rmfamily{MAPS~}}       % Meteoritics and Planetary Science

\usepackage{amsmath}
\usepackage{amssymb}

\def\Teff{$T_{\rm eff}$}
\def\Msun{{\rm M}_\odot}
\def\Rsun{{\rm R}_\odot}
\def\kms{\rm km~s$^{-1}$}

\def\arcsec{\hbox{$^{\hbox{\rlap{\hbox{\lower4pt\hbox{$\,\prime\prime$}}                         }\hbox{$\frown$}}}$}}

\newcommand{\msun}{$M_{\odot}$}
\newcommand{\etal}{{\it et al.}}


\newcommand{\half}{{\ensuremath{\textstyle\frac12}}}
\newcommand{\threehalf}{{\ensuremath{\textstyle\frac32}}}
\newcommand{\third}{{\ensuremath{\textstyle\frac13}}}
\newcommand{\quarter}{{\ensuremath{\textstyle\frac14}}}
\newcommand\apgt{\ {\raise-.5ex\hbox{$\buildrel>\over\sim$}}\ }
\newcommand\aplt{\ {\raise-.5ex\hbox{$\buildrel<\over\sim$}}\ }

\newcommand{\kin}{{\ensuremath K}}
\newcommand{\mbar}{{\ensuremath \langle m\rangle}}
\newcommand{\msun}{{\ensuremath M_\odot}}
\newcommand{\pot}{{\ensuremath U}}
\newcommand{\rvir}{{\ensuremath R_{vir}}}
\newcommand{\rh}{{\ensuremath R_h}}
\newcommand{\rj}{{\ensuremath R_J}}
\newcommand{\rsun}{{\ensuremath R_\odot}}
\newcommand{\tcc}{{\ensuremath t_{cc}}}
\newcommand{\tdis}{{\ensuremath t_{dis}}}
\newcommand{\tdyn}{{\ensuremath t_{dyn}}}
\newcommand{\tr}{{\ensuremath t_r}}
\newcommand{\tenc}{{\ensuremath t_{enc}}}
\newcommand{\trh}{{\ensuremath t_{rh}}}
\newcommand{\trl}{{\ensuremath t_{rl}}}
\newcommand{\tseg}{{\ensuremath t_{seg}}}
\newcommand{\vdisp}{{\ensuremath \langle v^2\rangle}}
\newcommand{\vrms}{{\ensuremath \vdisp^{1/2}}}
\newcommand{\vesc}{{\ensuremath v_{esc}}}
\newcommand{\vinf}{{\ensuremath v_\infty}}

\newcommand{\vv}{{\bf v}}
\newcommand{\vx}{{\bf x}}
\newcommand{\va}{{\bf a}}





